PhysDesignBench: Can AI Agents Perform Real-World Physics Engineering Design?

AI agents can increasingly write code, use engineering software, and complete complex workflows. But can they turn an engineering specification into a working physical design? Unlike conventional coding tasks, physics-based engineering design requires agents to navigate physical constraints, interpret simulation feedback, and iteratively improve solutions whose performance cannot be determined from code alone. We introduce PhysDesignBench, a benchmark of 26 end-to-end physics-based engineering tasks, comprising 16 open-ended Design tasks and 10 Reimplementation tasks based on published devices. Agents work with engineering software under limited time and simulation budgets, with their designs independently evaluated for physical validity and performance. Across 11 model-agent configurations, the highest overall normalized score is 0.474, while the highest engineering pass rate is only 19.2% (5 of 26 tasks). On open-ended Design tasks, the number of valid final submissions ranges from 2 to all 16 across configurations. Even when agents produce valid reimplementations, they rarely match published performance. We release the benchmark, evaluation harness, and accompanying resources at https://physdesignbench.com/, with plans to expand the task collection to support continued evaluation of autonomous engineering agents.

==> table/harness_ablation/totals.tex <==
\begin{tabular}{@{}l*{5}{c}@{}}
\toprule
\textcolor{AblationAccent}{\textbf{Agent}}
 & \textcolor{AblationAccent}{\textbf{Valid}}
 & \makecell{\textcolor{AblationAccent}{\textbf{Score}}\\(\%)}
 & \makecell{\textcolor{AblationAccent}{\textbf{Total time}}\\(min)}
 & \textcolor{AblationAccent}{\textbf{\makecell{Total\\probes}}}
 & \makecell{\textcolor{AblationAccent}{\textbf{Tokens}}\\(M)} \\
\midrule
\rowcolor{AblationTint}
\multicolumn{6}{@{}l}{\strut\textcolor{AblationAccent}{\textbf{GPT-6.1 Sol}}\enspace\textcolor{black!60}{(medium)}} \\
Codex & 12/16 & $\mathbf{39.3}\,\pm\,14.0$ & 119.7 & 22.1 & 21.22 \\
mini-SWE-agent & 12/16 & $37.9\,\pm\,12.6$ & 117.9 & 24.5 & \textbf{7.86} \\
\addlinespace[3pt]
\rowcolor{AblationTint}
\multicolumn{6}{@{}l}{\strut\textcolor{AblationAccent}{\textbf{Sonnet 5.5}}\enspace\textcolor{black!60}{(high)}} \\
Claude Code & 10/16 & $31.6\,\pm\,12.3$ & 95.4 & 23.0 & 21.87 \\
mini-SWE-agent & 10/16 & $\mathbf{34.1}\,\pm\,13.7$ & 95.6 & 21.2 & \textbf{13.56} \\
\bottomrule
\end{tabular}


==> table/main_results.tex <==
% Generated by plotting.export_main_table from the active main snapshot.
\begin{tabular}{@{}llccccc@{}}
\toprule
& & \multicolumn{2}{c}{Design} & \multicolumn{2}{c}{Reimplementation} & \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Model & Agent & Score & Valid & Score & Valid & Overall \\
\midrule
GPT-6 Astra & Codex & 0.510 & 16/16 & 0.417 & 10/10 & 0.474 \\
Opus 5.5 & Claude Code & 0.429 & 15/16 & 0.347 & 10/10 & 0.397 \\
GPT-6.1 Sol & Codex & 0.393 & 14/16 & 0.399 & 10/10 & 0.395 \\
Fable 5.1 & Claude Code & 0.326 & 13/16 & 0.348 & 10/10 & 0.334 \\
Sonnet 5.5 (high) & Claude Code & 0.316 & 11/16 & 0.328 & 10/10 & 0.321 \\
Gemini 4 Argon & mini-SWE-agent & 0.216 & 7/16 & 0.308 & 10/10 & 0.252 \\
Muse Wonder (high) & Muse Code & 0.172 & 7/16 & 0.353 & 10/10 & 0.242 \\
GPT-5.6 Sol & Codex & 0.195 & 10/16 & 0.295 & 10/10 & 0.233 \\
Kimi K3.1 Pro & Claude Code & 0.184 & 8/16 & 0.284 & 10/10 & 0.222 \\
GLM 5.3 Flash (max) & mini-SWE-agent & 0.098 & 3/16 & 0.236 & 10/10 & 0.151 \\
GLM 5.3 Flash (high) & Claude Code & 0.061 & 2/16 & 0.229 & 10/10 & 0.125 \\
\bottomrule
\end{tabular}


==> table/single_agent_task_results.tex <==
\color{black}
\begin{longtable}{@{}
    >{\raggedright\arraybackslash}p{0.38\textwidth}
    >{\centering\arraybackslash}p{0.07\textwidth}
    >{\centering\arraybackslash}p{0.11\textwidth}
    >{\raggedleft\arraybackslash}p{0.10\textwidth}
    >{\raggedleft\arraybackslash}p{0.10\textwidth}
    >{\raggedleft\arraybackslash}p{0.08\textwidth}@{}}
\caption{\color{black}Task-level outcomes for \texttt{gpt-5.6-sol-medium}. $J$ is the raw task objective, $S$ is the reference-relative score from Equation~\ref{eq:reporting-score}, and Probes is the number of diagnostic evaluator calls. U denotes an unavailable result and NR a result not reported.}
\label{tab:single-agent-task-results}\\
\toprule
Task & Track & Status & $J$ & $S$ & Probes \\
\midrule
\endfirsthead
\multicolumn{6}{l}{\small\itshape Table~\ref{tab:single-agent-task-results} continued}\\
\toprule
Task & Track & Status & $J$ & $S$ & Probes \\
\midrule
\endhead
\midrule
\multicolumn{6}{r}{\small\itshape Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot

90-degree SiN waveguide bend (v0) & D & Valid & 0.1144 & 1.2724 & 40 \\
Eight-delay MZI spectrometer (v1) & D & Valid & 0.4294 & 0.6776 & 40 \\
Eight-mode quantum projector (v2) & D & Valid & 10.3435 & 0.2444 & 31 \\
Four-mode quantum projector (v1) & D & Valid & 3.1171 & 0.4285 & 27 \\
Four-wavelength, four-port cross-connect (v2) & D & Invalid & -- & -- & 40 \\
Four-wavelength, two-port cross-connect (v1) & D & Invalid & -- & -- & 40 \\
Microresonator modulator (v1) & D & Valid & 0.0541 & 1.2495 & 40 \\
Microresonator modulator (v2) & D & Invalid & -- & -- & 18 \\
Microring-assisted Fourier spectrometer (v1) & D & Valid & 0.5346 & 0.8436 & 40 \\
MZI-coupled microring add-drop filter (v1) & D & Valid & 3.0237 & 0.5406 & 32 \\
MZI-coupled microring add-drop filter (v2) & D & Invalid & -- & -- & 40 \\
Rectangular MZI mesh (v1) & D & Valid & 0.4644 & 0.8121 & 13 \\
Rectangular MZI mesh (v2) & D & U & -- & -- & -- \\
Serial dual-ring-assisted MZI filter (v1) & D & Invalid & -- & -- & 31 \\
WDM channelizer (v1) & D & Valid & 16.3121 & 0.1918 & 13 \\
WDM channelizer (v2) & D & Valid & 32.7462 & 0.1313 & 9 \\

Anisotropic-SWG beamsplitter (v0) & I/O & Valid & 0.5655 & 1.2775 & 30 \\
$\alpha$-Si/SiN SWG grating coupler (v0) & I/O & NR & -- & -- & -- \\
Dual-trident SWG edge coupler (v0) & I/O & Valid & 0.5217 & 1.3143 & 30 \\
HMDM full circuit (v0) & I/O & NR & -- & -- & -- \\
Sb\textsubscript{2}Se\textsubscript{3}/Si polarization rotator (v0) & I/O & NR & -- & -- & -- \\
SRSN grating coupler (v0) & I/O & Valid & 1.2474 & 1.0468 & 30 \\
TFLN MMI crossing (v0) & I/O & NR & -- & -- & -- \\
TFLN polarization-insensitive MMI (v0) & I/O & NR & -- & -- & -- \\
TFLN slow-light modulator section (v0) & I/O & NR & -- & -- & -- \\
Trapezoidal-SWG 3-dB coupler (v0) & I/O & Valid & 2.7873 & 0.5281 & 30 \\

\end{longtable}


==> table/variance/tasks.tex <==
\begin{tabular}{lrrrrr}
\toprule
Task & v0 & v1 & v2 & Mean & SD \\
\midrule
90SiN Bend-v0 & 0.609 & 0.564 & 0.573 & 0.582 & 0.024 \\
MZI-Spec-8 & 0.465 & 0.484 & 0.467 & 0.472 & 0.010 \\
Quantum-4 & 0.518 & 0.501 & 0.501 & 0.507 & 0.010 \\
Quantum-8 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Ring-XC-v1 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Ring-XC-v2 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Microresonator-v1 & 0.650 & 0.663 & 0.733 & 0.682 & 0.045 \\
Microresonator-v2 & 0.514 & 0.537 & 0.518 & 0.523 & 0.013 \\
RAFT-Spec & 0.412 & 0.399 & 0.405 & 0.405 & 0.007 \\
MZI-Ring-v1 & 0.353 & 0.149 & 0.383 & 0.295 & 0.127 \\
MZI-Ring-v2 & 0.000 & 0.000 & 0.010 & 0.003 & 0.006 \\
MZI-v1 & 0.681 & 0.559 & 0.699 & 0.646 & 0.077 \\
MZI-v2 & 0.388 & 0.503 & 0.531 & 0.474 & 0.076 \\
Serial MZI-v1 & 0.000 & 0.051 & 0.043 & 0.031 & 0.027 \\
WDM-v1 & 0.133 & 0.080 & 0.343 & 0.185 & 0.139 \\
WDM-v2 & 0.340 & 0.117 & 0.000 & 0.152 & 0.173 \\
Anisotropic SWG-v0 & 0.599 & 0.628 & 0.569 & 0.599 & 0.030 \\
$\alpha$-Si/Si$_3$N$_4$ Grating-v0 & 0.266 & 0.236 & 0.236 & 0.246 & 0.017 \\
Dual-Trident SWG-v0 & 0.345 & 0.349 & 0.389 & 0.361 & 0.024 \\
HMDM polarization splitter--rotator & 0.104 & 0.103 & 0.092 & 0.100 & 0.007 \\
HMDM six-channel WDM & 0.028 & 0.032 & 0.019 & 0.026 & 0.007 \\
Sb$_2$Se$_3$/Si Rotator-v0 & 0.466 & 0.507 & 0.484 & 0.486 & 0.020 \\
SRSN Grating-v0 & 0.525 & 0.531 & 0.521 & 0.526 & 0.005 \\
TFLN Crossing-v0 & 0.297 & 0.347 & 0.246 & 0.297 & 0.051 \\
TFLN PI-MMI-v0 & 0.305 & 0.353 & 0.293 & 0.317 & 0.032 \\
Trapezoidal SWG-v0 & 0.349 & 0.194 & 0.325 & 0.289 & 0.083 \\
\bottomrule
\end{tabular}


==> working_examples/srsn_fable.tex <==
\subsection{Reimplementation: SRSN --- Claude Fable 5.1 / Claude Code}
\label{app:working-srsn_fable}
\begin{tcolorbox}[weouter,title={Task materials and recorded trajectory},title after break={Reimplementation: SRSN --- Claude Fable 5.1 / Claude Code (continued)}]
\noindent\textit{Budget: 120 minutes; 30 probes. Reasoning effort: medium.}\par\smallskip
\noindent\textbf{Materials available before the first agent turn.}\par
\begin{tcolorbox}[wecontext,title={instruction.md --- objective and supplied references}]
\begin{lstlisting}[style=wecode]
[...]
Implement the SRSN-on-SiN vertical grating coupler from the provided paper as
one final layout component. First reproduce the paper's Table-2 pattern and use
trusted probes to debug it; then optimize the permitted grating geometry for
coupling efficiency at `1550 nm`.
[...]
eta(1550 nm) = P_TE00_waveguide / P_incident_gaussian
J = -10 log10(eta(1550 nm))
[...]
- `references/s41598-026-44998-0.pdf`: source paper.
- `references/paper_parameters.json`: extracted stack, excitation,
  measurement, Table-2 geometry, and published results.
- `task_profile.json`: authoritative submission, layout, objective, and
  evaluation contract.
- `harness_contract.md`: source-freezing, probe, and final-verifier workflow.
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[wecontext,title={task\_profile.json and harness\_contract.md --- design variables and probes}]
\begin{lstlisting}[style=wecode]
[...]
"learner_controls": [
      "srsn_grating_polygons",
      "periods",
      "tooth_widths",
      "tooth_positions",
      "gaps",
      "chirp",
      "apodization",
      "bounded_tooth_count"
    ],
    "evaluator_controls": [
[...]
The sidecar freezes and hashes it, builds
fresh canonical GDS in the restricted non-root builder, validates the public
contract, runs the canonical evaluator, and writes and prints a unique
`/workspace/probe_results_N.json`.
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[wecontext,title={design.py --- editable starter}]
\begin{lstlisting}[style=wecode]
[...]
import photonforge as pf


def build_submission():
    """Return one PhotonForge component containing SRSN polygons on (1, 0)."""
    return pf.Component("SRSN_FINAL_GRATING")
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 2}]
I'll start by reading the task contract files and the extracted paper parameters.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 2}]
\begin{lstlisting}[style=wecode]
ls -la && cat task_profile.json && cat harness_contract.md && cat references/paper_parameters.json
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 2}]
\begin{lstlisting}[style=wecode]
[...]
"score_layer": [1, 0],
    "allowed_layers": [[1, 0]],
[...]
\end{lstlisting}
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 4}]
Baseline first: I'll write the Table-2 geometry into \texttt{design.py}, validate it locally, and then probe it.
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 6}]
\begin{lstlisting}[style=wecode]
time run_probe 2>&1 | tail -120
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 6}]
\begin{lstlisting}[style=wecode]
[...]
    "gate_pass": true,
[...]
    "probes_remaining": 29,
[...]
    "score": 1.2702447972441466,
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 7}]
Baseline probe: J = 1.27 dB (paper reports 1.37 dB), valid and only \textasciitilde{}15 s per probe. 29 probes remain. Let me check what local simulation tools I have for offline optimization before spending probes.
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 13}]
Sign error in the H-field curl updates caused the blow-up. Fixing and also tightening the inner loop for speed.
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 27}]
Run time is the culprit: 340 fs gave -1.05 dB vs -1.20 dB at 420 fs, so the result is not yet time-converged. Checking longer runs.
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 28}]
Converged to -1.222 dB for runs $\geq$500 fs at a 40 nm grid ($\approx$10 s per simulation). With 4 cores that's \textasciitilde{}24 evaluations/minute. Updating the evaluator settings and launching stage 1.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 28}]
\begin{lstlisting}[style=wecode]
[...]
s = open('evalpool.py').read()
s = s.replace('DX = 0.025\nT_TOTAL = 420.0', 'DX = 0.04\nT_TOTAL = 550.0\nSIM_KW = dict(x_min=-5.0, x_max=24.5, z_sub=0.6, z_air=1.0, npml=25, x_mon=-3.5)')
s = s.replace('_sim = fdtd2d.Sim(dx=DX)', '_sim = fdtd2d.Sim(dx=DX, **SIM_KW)')
[...]
\end{lstlisting}
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 34}]
Stage 2 is improving steadily (-1.224 $\to$ -1.158 dB in 2D after three iterations). I'll let it run and then probe an intermediate best to confirm the 2D gains transfer to the 3D evaluator.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 35}]
\begin{lstlisting}[style=wecode]
[...]
python write_design.py s2a_best.json
[...]
run_probe
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 35}]
\begin{lstlisting}[style=wecode]
wrote design.py with 20 teeth; 2D CE -1.0861532776396867
[...]
    "score": 1.1576268248549229,
[...]
            "valid": true
[...]
\end{lstlisting}
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 42}]
Now the probe-driven global scan on the 3D evaluator: scale all periods by a factor around the current best (J = 1.1454).
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 42}]
\begin{lstlisting}[style=wecode]
[...]
P = [p * scale_p for p in src["periods"]]
[...]
out = subprocess.run(["run_probe"], capture_output=True, text=True, cwd="/workspace").stdout
[...]
python probe_variant.py s3a_best.json 1.004 0.0 p_s1004; python probe_variant.py s3a_best.json 0.996 0.0 p_s0996
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 42}]
\begin{lstlisting}[style=wecode]
[...]
'scale_p': 1.004, 'dw': 0.0, 'score': 1.130506042973096, 'valid': True
[...]
'scale_p': 0.996, 'dw': 0.0, 'score': 1.3708823246256303, 'valid': True
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 43}]
Scaling periods up by 0.4\% improved the 3D score to 1.1305 dB (scaling down hurt badly). Continuing the scan upward.
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 58}]
The file is clean and self-contained. With 8 probes and \textasciitilde{}30 minutes left, I'll try one more low-risk 3D knob (tail tooth widths only), keeping the verified best as fallback.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 58}]
\begin{lstlisting}[style=wecode]
[...]
P = list(src["periods"]); W = [w + (dw if i >= i0 else 0.0) for i, w in enumerate(src["widths"])]
[...]
python probe_tail.py p_s3c_s10015.json 0.02 14 p_tail_p20; python probe_tail.py p_s3c_s10015.json -0.02 14 p_tail_m20
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 58}]
\begin{lstlisting}[style=wecode]
{'tag': 'p_tail_p20', 'src': 'p_s3c_s10015.json', 'dw_tail': 0.02, 'i0': 14, 'score': 1.112029199740468, 'valid': True, 'remaining': 7}
{'tag': 'p_tail_m20', 'src': 'p_s3c_s10015.json', 'dw_tail': -0.02, 'i0': 14, 'score': 1.096115098801538, 'valid': True, 'remaining': 6}
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 59}]
Narrower tail teeth helped (1.0961 dB). Pushing further.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 59}]
\begin{lstlisting}[style=wecode]
python probe_tail.py p_s3c_s10015.json -0.04 14 p_tail_m40; benchmark_status | grep remaining
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 59}]
\begin{lstlisting}[style=wecode]
{'tag': 'p_tail_m40', 'src': 'p_s3c_s10015.json', 'dw_tail': -0.04, 'i0': 14, 'score': 1.1067330905189445, 'valid': True, 'remaining': 5}
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weagent,title={Agent --- step 60}]
The -0.04 $\mu$m offset is worse, so -0.02 $\mu$m is the optimum. Installing that design as final and confirming with a probe of the exact file.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 60}]
\begin{lstlisting}[style=wecode]
python write_design.py p_tail_m20.json
[...]
run_probe
[...]
sha256sum design.py
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 60}]
\begin{lstlisting}[style=wecode]
[...]
    "score": 1.096115098801538,
    "submission_sha256": "517889c4b7a51d695097b1b41f92cfef87a353f49e5b052cc745e27fefa96a78",
            "valid": true
[...]
\end{lstlisting}
\end{tcolorbox}
\weomitted
\begin{tcolorbox}[weagent,title={Agent --- step 62}]
Neither beats 1.0961 dB. Restoring the verified best as the final submission and checking its hash.
\end{tcolorbox}
\begin{tcolorbox}[wetool,title={Tool call: Bash --- step 62}]
\begin{lstlisting}[style=wecode]
cp /workspace/opt/best_design_1.0961.py /workspace/design.py && sha256sum /workspace/design.py
[...]
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[weresponse,title={Tool response --- step 62}]
\begin{lstlisting}[style=wecode]
517889c4b7a51d695097b1b41f92cfef87a353f49e5b052cc745e27fefa96a78  /workspace/design.py
[...]
\end{lstlisting}
\end{tcolorbox}
\par\noindent\begin{minipage}{\linewidth}
\weomitted
\begin{tcolorbox}[weagent,title={Final agent response --- step 64}]
The work is complete and the final submission is in place. Here is the summary.

\smallskip
\textbf{Result}

\smallskip
\texttt{/workspace/design.py} holds a 20-tooth SRSN grating whose coupling loss on the trusted 3D evaluator is \textbf{J = 1.096 dB} (CE = -1.096 dB), confirmed by a probe of the exact final file (sha256 \texttt{517889c4\ldots{}}). That is 0.17 dB better than the paper's Table-2 geometry as evaluated by the same harness (J = 1.270 dB) and 0.27 dB better than the paper's published 3D figure (1.37 dB). The layout passes every geometry rule: 20 rectangles on layer (1, 0), minimum tooth 0.205 $\mu$m, minimum gap 0.206 $\mu$m, grating from x = 0.83 to 19.13 $\mu$m, width exactly 14 $\mu$m centered on y = 0.
[...]
- A physics observation that shaped the design: at vertical incidence the grating is also a second-order Bragg reflector, so the uniform tail reflects wrongly-launched (+x) light back toward the waveguide; removing tail teeth costs up to 0.08 dB.
[...]
\end{tcolorbox}
\begin{tcolorbox}[wefinal,title={Independent final evaluation}]
The frozen submission passes the native final gates. The independently rebuilt final gives $J=1.096115\,\mathrm{dB}$ and $S=0.555530$ on the paper's 0--1 scale. Its source hash matches the exact-file confirmations in probes 24 and 26.
\end{tcolorbox}
\begin{center}\includegraphics[width=.40\linewidth]{working_examples/srsn_fable_final.pdf}\par
{\footnotesize Original GDS from the independent final evaluation.}\end{center}
\end{minipage}
\end{tcolorbox}

